Pointwise Maximal Leakage on General Alphabets

Pointwise maximal leakage (PML) is an operationally meaningful privacy measure that quantifies the amount of information leaking about a secret $X$ to a single outcome of a related random variable $Y$. In this paper, we extend the notion of PML to random variables on arbitrary probability spaces. We develop two new definitions: First, we extend PML to countably infinite random variables by considering adversaries who aim to guess the value of discrete (finite or countably infinite) functions of $X$. Then, we consider adversaries who construct estimates of $X$ that maximize the expected value of their corresponding gain functions. We use this latter setup to introduce a highly versatile form of PML that captures many scenarios of practical interest whose definition requires no assumptions about the underlying probability spaces.

==> sections/current/properties.tex <==
\section{Properties}
\label{sec:properties}

Properties inherited by $D_{\infty}(P\parallel Q)$~\cite{van2014renyi}
\begin{itemize}
    \item convex in $Q$
    \item jointly quasi-convex in $(P, Q)$
    \item Data Processing Inequality (pre-processing)
\end{itemize}

==> sections/current/removed.tex <==
\section{Definitions and properties}
We recall the definition of PML as stated in. Underlying probability space is $(\Omega, \mathcal A, \mathbb P)$. 

\begin{definition}[Pointwise maximal leakage]
Let $P_{XY}$ denote the joint distribution of $X$ and $Y$, and suppose the Markov chain $U - X - Y - \hat{U}$ holds. The pointwise maximal leakage from $X$ to $y \in \mathrm{supp}(P_Y)$, $\ell_{P_{XY}}(X \to y)$, is defined as 
\begin{align}
\begin{split}
\label{eq:privacy_rv_def}
    \ell_{P_{XY}}(X\to y) &\coloneqq \sup_{P_{U \mid X}} \ell_U(X\to y) \\
    &= \log \sup_{P_{U \mid X}} \frac{\sup_{P_{\hat U \mid Y=y}} \mathbb P \left[U=\hat U \mid Y=y \right]}{\max_{u 
    \in \mathcal{U}} P_U(u)}.
\end{split}
\end{align}
\end{definition}

Similarly to~\cite[Lemma 1]{issa2019operational} for ML, we show that PML verifies data-process inequality.

\begin{lemma}
For any joint distribution $P_{XY}$, 
if the Markov chain $X-Y-Z$ holds, $$\ell_{P_{XZ}}(X\to z)\leq \ell_{P_{XY}}(X\to y).$$

\begin{IEEEproof}
Consider any discrete $U$ satisfying $U-X-Y-Z$, then
\begin{align}
\begin{split}
\ell_U(X\to z)&= \log  \frac{\sup_{P_{\hat U \mid Z=z}} \mathbb P \left[U=\hat U(Z) \mid Z=z \right]}{\max_{u 
    \in \mathcal{U}} P_U(u)}\\
    &=\log  \frac{\sup_{P_{\hat U \mid Z(Y)=z}} \mathbb P \left[U=\hat U(Z(Y)) \mid Z(Y)=z \right]}{\max_{u 
    \in \mathcal{U}} P_U(u)}\\
    & \leq \log  \frac{\sup_{P_{\hat U \mid Y=y}} \mathbb P \left[U=\hat U(Y) \mid Y=y \right]}{\max_{u 
    \in \mathcal{U}} P_U(u)}=\ell_U(X\to y),
\end{split}
\end{align}hence implying 
\begin{align}
    \ell_{P_{XZ}}(X\to z)=
    \sup_{P_{U \mid X}} \ell_U(X\to z) \leq
     \sup_{P_{U \mid X}} \ell_U(X\to z) = \ell_{P_{XY}}(X\to y).
\end{align}

\todo[inline]{Check other properties}
Similarly $\ell_{P_{XZ}}(X\to z) \leq \ell_{P_{YZ}}(Y\to z)$??
\end{IEEEproof}
\end{lemma}


\section{TodoList}
\begin{enumerate}
    \item check when you can swap lim and inf (unit convergence)
    \item when is the kernel absolutely continous wrt the marginal?
    \item Data-process inequality for PML
    \item Properties of general maximal leakage 
\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
First, we show that the LHS of~\eqref{eq:countable_thm} lower bounds the RHS. Fix a random variable $U$ induced by some kernel $P_{U \mid X}$. We write 
\begin{align*}
    \ell_U (X \to Y) &= \frac{\sup_{P_{\hat U \mid Y}} \mathbb P \left[ U = \hat U \mid \sigma(Y) \right]}{\max_{u} P_U(u)}\\[0.5em]
    &= \frac{\sup_{P_{\hat U \mid Y}} \sum_{u, \hat u} P_{U \mid Y} (u) \; P_{\hat U \mid Y}(\hat u) \; \mathds{1}(u=\hat u)}{\max_{u} P_U(u)}\\[0.5em]
    &= \frac{\sup_{P_{\hat U \mid Y}} \sum_{u} P_{U \mid Y} (u) \; P_{\hat U \mid Y}(u)}{\max_{u} P_U(u)}\\[0.5em]
    &\leq \frac{\max_u P_{U \mid Y} (u) }{\max_{u} P_U(u)}\\[0.5em]
    &= \frac{\max_{u} \sum_x P_{U \mid X=x}(x) \; P_{X \mid Y} (x)}{\max_u P_{U}(u)}\\
    &= \max_u \sum_x  P_{X \mid U=u}(x) \cdot \frac{P_{X \mid Y}(x)}{P_X(x)} \cdot \frac{P_U(u)}{\max_{u'} P_U(u')}\\
    &\leq \max_u \sum_x  P_{X \mid U=u}(x) \; \frac{P_{X \mid Y}(x)}{P_X(x)}\\
    &\leq \sup_x \frac{P_{X \mid Y}(x)}{P_X(x)}. 
\end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
